Astronomers and the Science Citation Index, 1981--1997

The Institute for Science Information (ISI) has generated two lists of citation information for astronomers that are uniquely restricted both as to the years surveyed for the cited papers, and the years surveyed for the citing papers. The main list gives citation data for 62,813 physicists and astronomers whose journal papers were cited 100 times or more from 1981.0 to 1997.5 by papers published during the same time interval. The second list gives the 200 most-cited papers/year published in refereed astronomical journals from 1981-1996, as cited in papers in those same journals from 1981.0-1998.0. Astronomer names were selected from various sources. From this work an Astronomy Citation Database (ACD) has been constructed, containing citation data for 6458+ astronomers, plus additional data for 173 astronomers and the top-10 cited papers published 1981-1996. Various problems, both substantial and subtle, of producing a reasonably fair citation database are detailed. Chief among these are whether to assign either parital or full credit for each author on a given paper. Whether one is honored with one of the top astronomy lifetime-awards is a strong function of how well your work stands out as your own, and in what kind of publications you publish (e.g., the ISI does not keep track of papers in meeting proceedings/books/catalogs). Name confusion affects this kind of analysis to the extent that that it would take an enormous effort to disentangle its effects and, even then, not all name confusion would be settled. A ``modest proposal'' is made that our professional field (and others) go to a system of uniquely associating an identification number to each author on each paper to solve the name confusion problem.

==> ACD_020100_top10papers <==
%auto-ignore
 627   13  1 Pringle, JE                                                          1981   ARA&A       19  137
 603   16  2 Vernazza, JE, Avrett, EH, & Loeser, R                                1981   ApJS        45  635
 473   30  3 Renzini, A & Voli, M                                                 1981   A&A         94  175
 466   33  4 Kutner, ML & Ulrich, BL                                              1981   ApJ        250  341
 431   42  5 Ostriker, JP & Cowie, LL                                             1981   ApJL       243  127
 398   51  6 Larson, RB                                                           1981   MNRAS      194  809
 395   53  7 Baldwin, JA, Phillips, MM, Terlevich, R                              1981   PASP        93    5
 382   55  8 Kwan, J & Krolik, JH                                                 1981   ApJ        250  478
 372   60  9 Fisher, JR & Tully, RB                                               1981   ApJS        47  139
 370   62 10 Vanderhucht, KA, Conti, PS, Lundstrom, I, & Stenholm, B              1981   SSRv        28  227
1100    1  1 Burstein, D & Heiles, C                                              1982   AJ          87 1165
 634   12  2 Elias, JE, Frogel, JA, Matthews, K & Neugebauer, G.                  1982   AJ          87 1029
 449   38  3 Scargle, JD                                                          1982   ApJ        263  835
 419   46  4 Graham, JA                                                           1982   PASP        94  244
 362   65  5 Sandage, A                                                           1982   ApJ        252  553
 338   74  6 Malkan, MA & Sargent, WLW                                            1982   ApJ        254   22
 325   79  7 Condon, JJ, Condon, MA, Gisler, G & Puschell, JJ                     1982   ApJ        252  102
 314   85  8 Blandford, RD & Payne, DG                                            1982   MNRAS      199  883
 311   89  9 Smith, BA, et al.                                                    1982   Sci        215  504
 297  106 10 Piccinotti, G, et al.                                                1982   ApJ        253  485
 826    4  1 Landolt, AU                                                          1983   AJ          88  853
 726    7  2 Iben, I, Jr & Renzini, A                                             1983   ARA&A       21  271
 696    8  3 Davis, M & Peebles, PJE                                              1983   ApJ        267  465
 682    9  4 Morrison, R & McCammon, D                                            1983   ApJ        270  119
 474   28  5 Bally, J & Lada, CJ                                                  1983   ApJ        265  824
 468   32  6 Schmidt, M & Green RF                                                1983   ApJ        269  352
 463   34  7 Bahcall, NA & Soniera, RM                                            1983   ApJ        270   20
 457   37  8 Kennicutt, RC, Jr                                                    1983   ApJ        272   54
 445   39  9 Huchra, JP, Davis, M, Latham, D, & Tonry, J                          1983   ApJS        52   89
 440   40 10 Hildebrand, RH                                                       1983   QJRAS       24  267
 617   14  1 Burstein, D & Heiles, C                                              1984   ApJS        54   33
 576   17  2 Yang, J, Turner, MS, Schramm, DN, Steigman, G, & Olive, KA           1984   ApJ        281  493
 527   21  3 Patterson, J                                                         1984   ApJS        54  443
 516   22  4 Leger, A & Puget, JL                                                 1984   A&A        137    5
 462   35  5 Zinn, R & West, MJ                                                   1984   ApJS        55   45
 461   36  6 Blumenthal, GR, Faber, SM, Primack, JR, Rees, MJ                     1984   Natur      311  517
 434   41  7 Jones, C & Forman, W                                                 1984   ApJ        276   38
 408   48  8 Bridle, AH, Perley, RA                                               1984   ARA&A       22  319
 405   49  9 Rees, MJ                                                             1984   ARA&A       22  471
 359   68 10 Kaiser, N                                                            1984   ApJL       284    9
 980    2  1 Draine, BT & Lee, HM                                                 1985   ApJ        285   89
 642   10  2 Davis, M, Efstathiou, G, Frenk, CS, & White, SDM                     1985   ApJ        292  371
 547   18  3 Rieke, GH & Lebofsky, MJ                                             1985   ApJ        288  618
 532   20  4 Antonucci, RRJ & Miller, JS                                          1985   ApJ        297  621
 495   25  5 Zinn, R                                                              1985   ApJ        292  424
 474   28  6 Lada, CJ                                                             1985   ARA&A       23  267
 412   47  7 VandenBerg, DA                                                       1985   ApJS        58  711
 404   50  8 Boesgaard, AM & Steigman, G                                          1985   ARA&A       23  319
 377   56  9 VandenBerg, DA & Bell, RA                                            1985   ApJS        58  561
 371   61 10 Knapp, GR & Morris, M                                                1985   ApJ        292  640
 769    6  1 Bardeen, JM, Bond, JR, Kaiser, N, & Szalay, AS                       1986   ApJ        304   15
 500   24  2 deLapparent, V, Geller, MJ, Huchra, JP                               1986   ApJL       302    1
 481   27  3 Mikheyev, SP & Smirnov, AY                                           1986   NUOV CIM C   9   17
 376   57  4 Woosley, SE & Weaver, TA                                             1986   ARA&A       24  205
 356   70  5 Barnes, J & Hut, P                                                   1986   Natur      324  446
 318   82  6 Dekel, A & Silk, J                                                   1986   ApJ        303   39
 291  113  7 Green, RF, Schmidt, M, & Liebert, J                                  1986   ApJS        61  305
 288  115  8 Paczynski, B                                                         1986   ApJ        304    1
 282  120  9 Aaronson, M, et al.                                                  1986   ApJ        302  536
 265  145 10 Horne, K                                                             1986   PASP        98  609
 636   11  1 Hedin, AE                                                            1987   J GEO R-S P 92 4649
 606   15  2 Shu, FM, Adams, FC, Lizano, S                                        1987   ARA&A       25   23
 374   58  3 Adams, FC, Lada, CJ, Shu, FH                                         1987   ApJ        312  788
 367   63  4 Heppner, JP & Maynard, NC                                            1987   J GEO R-S P 92 4467
 309   92  5 Dame, TM et al.                                                      1987   ApJ        322  706
 306   94  6 Veilleux, S & Osterbrock, DE                                         1987   ApJS        63  295
 283  119  7 Hewitt, A & Burbidge, G                                              1987   ApJS        63    1
 280  124  8 Tsyganenko, NA                                                       1987   P&SS        35 1347
 275  130  9 Blake, GA, Sutton, EC, Masson, CR & Phillips, TG                     1987   ApJ        315  621
 274  132 10 Maeder, A & Meynet, G                                                1987   A&A        182  243
 825    5  1 Stetson, PB                                                          1988   PASP        99  191
 428   43  2 Tyson, JA                                                            1988   AJ          96    1
 421   44  3 Lyndenbell, D, et al.                                                1988   ApJ        326   19
 420   45  4 Sanders, DB, et al.                                                  1988   ApJ        325   74
 318   82  5 Maeder, A & Meynet, G                                                1988   A&AS        76  411
 294  109  6 Efstathiou, G, Ellis, RS, & Peterson, BA                             1988   MNRAS      232  431
 271  137  7 Broadhurst, TJ, Ellis, RS, & Shanks, T                               1988   MNRAS      235  827
 267  142  8 Bertout, C, Basri, G, & Bouvier, J                                   1988   ApJ        330  350
 260  154  9 van Dishoeck, EF, Ewine, F, & Black, JH                              1988   ApJ        334  771
 230  205 10 Lightman, AP & White, TR                                             1988   ApJ        335   57
 485   26  1 Cardelli, JA, Clayton, GC, & Mathis, JS                              1989   ApJ        345  245
 361   66  2 Barthel, PD                                                          1989   ApJ        336  606
 352   72  3 Wheeler, JC, Sneden, C, & Truran, JW, Jr                             1989   ARA&A       27  279
 337   76  4 Abell, GO, Corwin, HG, Jr, & Olowin, RP                              1989   ApJS        70    1
 314   85  5 Geller, MJ & Huchra, JP                                              1989   Sci        246  897
 305   95  6 Turner, TJ & Pounds, KA                                              1989   MNRAS      240  833
 299  102  7 Kennicutt, RC, Jr                                                    1989   ApJ        344  685
 298  103  8 Turner, MJL, et al.                                                  1989   PASJ        41  345
 264  149  9 Taylor, JH & Weisberg, JM                                            1989   ApJ        345  434
 263  151 10 Tsyganenko, NA                                                       1989   P&SS        37    5
 373   59  1 Beckwith, SVW, Sargent, AI, Chini, RS, & Guesten, R                  1990   AJ          99  924
 322   80  2 Broadhurst, TJ, Ellis, RS, Koo, DC, & Szalay, AS                     1990   Natur      343  726
 303   99  3 Maddox, SJ, Efstathiou, G, Sutherland, WJ, & Loveday, J              1990   MNRAS      242   43
 293  110  4 Mathis, JS                                                           1990   ARA&A       28   37
 273  135  5 Mather, JC, et al.                                                   1990   ApJL       354   37
 265  145  6 Dickey, JM & Lockman, FJ                                             1990   ARA&A       28  215
 239  188  7 Pounds, KA, Nandra, K, Stewart, GC, George, GC & Fabian, AC          1990   Natur      344  132
 238  189  8 Gioia, IM, et al.                                                    1990   ApJS        72  567
 217  243  9 Colless, M, Ellis, RS, Taylor, K, & Hook, RN                         1990   MNRAS      244  408
 215  246 10 Maeder, A                                                            1990   A&AS        84  139
 541   19  1 Walker, TP, Steigman, G, Kang, HS, Schramm, DM, & Olive, KA          1991   ApJ        376   51
 281  122  2 Morton, DC                                                           1991   ApJS        77  119
 249  175  3 Saunders, W, Frenk, C, Rowan-Robinson, M, Lawrence, A, Efstathiou, G 1991   Natur      349   32
 235  196  4 Stocke, JT, et al.                                                   1991   ApJS        76  813
 227  213  5 Duquennoy, A & Mayor, M                                              1991   A&A        248  485
 227  213  5 Tsuneta, S, et al.                                                   1991   SoPh       136   37
 212  257  7 Lilly, SJ, Cowie, LL, & Gardner, JP                                  1991   ApJ        369   79
 211  259  8 Balbus, SA  & Hawley, JF                                             1991   ApJ        376  214
 179  378  9 Clavel, J, et al.                                                    1991   ApJ        366   64
 173  413 10 George, IM  & Fabian, AC                                             1991   MNRAS      249  352
 903    3  1 Smoot, GF, et al.                                                    1992   ApJL       396    1
 510   23  2 Landolt, AU                                                          1992   AJ         104  340
 473   30  3 Schaller, G, Schaerer, D, Meynet, G, & Maeder, A                     1992   A&AS        96  269
 398   51  4 Stark, AA, et al.                                                    1992   ApJS        79   77
 309   92  5 Rogers, FJ  & Iglesias, CA                                           1992   ApJS        79  507
 292  111  6 Wright, EL, et al.                                                   1992   ApJL       396   13
 277  127  7 Meegan, CA, et al.                                                   1992   Natur      355  143
 220  234  8 Iglesias, CA, Rogers, FJ,  & Wilson, BG                              1992   ApJ        397  717
 219  236  9 Loveday, J, Peterson, BA, Efstathiou, G, & Maddox, SJ                1992   ApJ        390  338
 214  250 10 Jacoby, GH, et al.                                                   1992   PASP       104  599
 297  106  1 Antonucci, R                                                         1993   ARA&A       31  473
 278  126  2 Alcock, C, et al.                                                    1993   Natur      365  621
 275  130  3 Edvardsson, B, et al.                                                1993   A&A        275  101
 261  153  4 Taylor, JH, Manchester, N, & Lyne, AG                                1993   ApJS        88  529
 215  246  5 Bruzual, G & Charlot, S                                              1993   ApJ        405  538
 190  319  6 White, SDM, Navarro, JF, Evrard, AE, & Frenk, CA                     1993   Natur      366  429
 186  338  7 Taylor, JH  & Cordes, JM                                             1993   ApJ        411  674
 172  416  8 Pounds, KA, et al.                                                   1993   MNRAS      260   77
 164  469  9 Klypin, A, Holtzman, J, Primack, J, & Regos, E                       1993   ApJ        416    1
 146  612 10 White, SDM,  Efstathiou, G, & Frenk, CA                              1993   MNRAS      262 1023
 242  184  1 Freedman, WL, et al.                                                 1994   Natur      371  757
 241  185  2 Tanaka, Y, Inoue, H, & Holt, SS                                      1994   PASL        46   37
 186  338  3 Lyne, AG  & Lorimer, DR                                              1994   Natur      369  127
 166  454  4 Mather, JC, et al.                                                   1994   ApJ        420  439
 158  512  5 Fichtel, CE, et al.                                                  1994   ApJS        94  551
 153  545  6 D'Antona, F  & Mazzitelli, I                                         1994   ApJS        90  467
 153  545  6 Songaila, A, Cowie, LL, Hogan, CJ, & Rugers, M                       1994   Natur      368  599
 152  560  8 Peacock, JA  & Dodds, SJ                                             1994   MNRAS      267 1020
 141  660  9 Nandra, K  & Pounds, KA                                              1994   MNRAS      268  405
 139  693 10 Bennett, CL, et al.                                                  1994   ApJ        436  423
 134  745  1 Von Montigny, C, et al.                                              1995   ApJ        440  525
 128  822  2 Copi, CJ, Schramm, DN, & Turner, MS                                  1995   Sci        267  192
 127  837  3 Hotlzman, JA, et al.                                                 1995   PASP       107 1065
 127  837  3 Thompson, DJ, et al.                                                 1995   ApJS       101  259
 110 1189  5 Miyoshi, M, et al.                                                   1995   Natur      373  127
 108 1239  6 Leitherer, C & Heckman, TM                                           1995   ApJS        96    9
  98 1484  7 Mayor, M  & Queloz, D                                                1995   Natur      378  355
  93 1638  8 Lilly, SJ, Tresse, L, Hammer, F, Crampton, D, & Le Fevre, O          1995   ApJ        455  108
  92 1668  9 Woosley, SE  & Weaver, TA                                            1995   ApJS       101  181
  87      10 Timmes, FX, Woosley, SE, & Weaver, TA                                1995   ApJS        98  617
  80       1 Steidel, CC, Giavalisco, M, Pettini, M, Dickinson, M, Adelberger, KL 1996   ApJL       462   17
  66       2 Tytler, D, Fan, X-M, & Burles, S                                     1996   Natur      381  207
  47       3 Ellis, RS, Colless, M, Broadhurst, T, Heyl, J & Glazebrook, K        1996   MNRAS      280  235
  47       3 Rugers, M  & Hogan, CJ                                               1996   ApJL       459    1
  45       5 Narayan, R, McClintock, JE, & Yi, I                                  1996   ApJ        457  821
  44       6 Babul, A  & Ferguson, HC                                             1996   ApJ        458  100
  43       7 Marcy, GW  & Butler, RP                                              1996   ApJ        464  147
  42       8 Navarro, JF, Frenk, CS, White, SDM                                   1996   ApJ        462  563
  42       8 Williams, RE, et al.                                                 1996   AJ         112 1335
  40      10 Alcock, C, et al.                                                    1996   ApJ        461   84
  40      10 Chaboyer, B, DeMarque, P, & Sarajedini, A                            1996   ApJ        459  558
  40      10 Hernquist, L, Katz, N, Weinberg, DH, \& Miralda-Escude', J           1996   ApJL       457   51  

